Deep Manifold Traversal: Changing Labels with Convolutional Features

Many tasks in computer vision can be cast as a "label changing" problem, where the goal is to make a semantic change to the appearance of an image or some subject in an image in order to alter the class membership. Although successful task-specific methods have been developed for some label changing applications, to date no general purpose method exists. Motivated by this we propose deep manifold traversal, a method that addresses the problem in its most general form: it first approximates the manifold of natural images then morphs a test image along a traversal path away from a source class and towards a target class while staying near the manifold throughout. The resulting algorithm is surprisingly effective and versatile. It is completely data driven, requiring only an example set of images from the desired source and target domains. We demonstrate deep manifold traversal on highly diverse label changing tasks: changing an individual's appearance (age and hair color), changing the season of an outdoor image, and transforming a city skyline towards nighttime.

==> colorization_text.tex <==
%!TEX root=main.tex
\paragraph{Semantic understanding.}
\label{ref:colorization}

Correct colorization of a grayscale image requires understanding semantic cues. Can our method colorize the face? The target domain is images annotated as ``color photo''. Although the attribute label is ``color photo'', the target domain is actually color faces since PCA projects out features unrelated to faces. Due to the scarcity of grayscale images, we only use 200 images in the source domain. In figure~\ref{fig:color}, we present results for four celebrities which do not have any color images in LFW.

Our method produced the correct skin tone for all four celebrities and the colorization is mostly constrained to the face. Clothing, background, ears, and hair are less colorized. No changes are made to facial structure, age, facial expression, and hairstyle. Our method learns to target the face -- supervised masks of facial regions are not used during training.
This experiment demonstrates that the changes made \emph{preserve information irrelevant to the change}.
Furthermore, the skin tone domain is clearly multimodal and our method correctly seeks nearby modes rather than merely moving toward a global mean image in the target domain.

\begin{wrapfigure}{R}{0.5\textwidth}
%\begin{figure*}[tb]
\begin{center}
\vspace{-8ex}
\centerline{\includegraphics[width=0.5\textwidth]{figures/colorization.pdf}}
\vspace{-2ex}
\caption{\textbf{Top row:} Input grayscale images. \textbf{Bottom row:} Targeted colorization of the face with correct skin tone by seeking a mode of the multimodal target domain. We do not use masks to target the face -- the targeting is learned unsupervised. Zoom in for details.}
%Privacy and utility for both Spearman's $\rho$ and Kendall's $\tau$.}
\vspace{-5ex}
\label{fig:color}
\end{center}
%\end{figure*}
\end{wrapfigure}

==> intro2.tex <==
%!TEX root=main.tex
\section{Introduction}


Many tasks in computer vision can be cast as a \emph{label changing} problem: given an input image, change the label of that image from some label $y^{s}$ to some target label $y^{t}$.
%Changing the class of an image is an important problem. Methods exist for semantic colorization \cite{chia2011semantic} and  of a grayscale image into a color image, ,  and  Images of faces, in
%particular, have attracted much attention. Methods have been proposed
%to
%synthesize new expressions \cite{kemelmacher2013internet},
%make a face older \cite{kemelmacher2014illumination},
%produce a high-quality face from a degraded image \cite{kolouri2015transport,duong2015beyond},
%manipulate hairstyles \cite{chai2012single},
%and change identity \cite{bitouk2008face}. What these recent works have in common is that they use domain-specific information or manual annotation to solve a specific task very well. In contrast, our method is general purpose and can be applied to many of these tasks.
 Examples of this general task include changing hairstyles and expressions \cite{chai2012single,kemelmacher2013internet}, example-based image colorization \cite{irony2005colorization,gupta2012image}, aging of faces \cite{kemelmacher2014illumination}, editing of outdoor scenes \cite{laffont2014transient} changing seasons \cite{neubert2013appearance}, and image morphs \cite{liao2014automating}, relighting a photo \cite{kopf2008deep,laffont2012coherent} and  hallucinating a night image from a day image \cite{shih2013data} among many others. A variety of specialized algorithms exist for each of these tasks. However, these algorithms often incorporate substantial domain-specific prior knowledge relevant to the task and may require hand annotation of images, rendering them unable to perform any other task. For example, it is unlikely that a facial aging algorithm would be able to change the season of an outdoor scene.

This motivates research into the most \emph{general} form of changing image appearances.  
A given image could be changed into a target image through linear interpolation in pixel space. However, intermediate images would not be meaningful because the set of natural images does not span a linear subspace in the pixel space. Instead, it is believed to constitute a low dimensional sub-manifold~\cite{weinberger2006unsupervised}. In order to make meaningful changes, the image traversal path must be confined to the underlying manifold throughout. 

Bengio et al. 2012 \cite{bengio2012better} suggests that deep convolutional networks simplify the manifold of natural images by learning a high level feature representation.  This suggests that deep learning is a natural choice for solving the label changing problem. However, recent work \cite{szegedy2013intriguing,nguyen2014deep} has demonstrated that this problem can be surprisingly hard for images. In the context of object classification with convolutional neural networks, it has been shown possible to change the \emph{prediction} of an image with tiny alterations that can be \emph{imperceptible to humans}, but such changes do not change the appearance of the image leave the class label untouched~\cite{szegedy2013intriguing}.
% \emph{class label}--the semantic ground truth~\cite{}.
% By altering class label, we really mean to change the intrinsic properties of the instance to another category.
In fact, the problem of changing class labels persists for most machine learning algorithms beyond deep learning~\cite{goodfellow2014explaining}.

In this paper we investigate how to make \emph{meaningful changes} to inputs in order to \emph{truly} change their class label. Formally, we are given training inputs from two classes: $\bx^{s}_1,\dots,\bx^{s}_m$ -- all of which are labeled as the \emph{source} class $y^{s}$, and $\bx^{t}_1,\dots,\bx^{t}_n$ -- all of which are labeled as the \emph{target} class $y^{t}$. Given a test input $\bbx^{s}$ from class $y^{s}$,  we would like to find a transformation $\bbx^{s}\!\rightarrow\! \bbx^{t}$, so that $\bbx^{t}$ is the $y^{t}$-transformed version of $\bbx^{s}$.
% is most similar to the original $\bbx^{s}$, yet associates with a class label of $y^{t}$ instead of $y^{s}$.
 


Our goal is to make semantic changes to images. What does this mean? This means we want to move along a manifold of natural images until we change the class of the image. Staying on the manifold is important since implausible and nonsense images are outside the manifold. Machine learning methods learn manifold so they would be a natural choice for manifold traversal. However, machine learning methods are susceptible to falling off the manifold easily~\cite{szegedy2013intriguing}. Addressing this problem is of central importance.

One interpretation of the results by Szegedy et al., 2014 \cite{szegedy2013intriguing} is that if we allow arbitrary movements off the manifold, we can find pockets in space that are associated with any arbitrary label. For example, one could change the \emph{predicted label} of an image of a zebra into a car by drawing imperceptibly faint signature features of cars on top of the zebra. 

\paragraph{Manifold Traversal.} 
For high-dimensional data to be interesting it must contain low-dimensional structure. Although embedded in very high-dimensional pixel spaces, natural images are believed to lie on lower dimensional sub-manifolds~\cite{weinberger2006unsupervised}. 


%Moving along image manifolds is challenging for at least two reasons: First, small changes across multiple dimensions tend to add up to large distances overall, making it easy to leave the manifold in high dimensional spaces; Second, we need to move $\bbx^{s}$ \emph{along the manifold} into a region where the class label $y^{t}$ is dominant. We address each of these points.

Inspired by an hypothesis in recent work by Bengio et al. 2012 \cite{bengio2012better}, we utilize a deep convolutional network trained on 1.2 million images~\cite{simonyan2014very} to simplify the manifold of natural images to a linear feature space. 
 by mapping images into a high level feature space, $\bbz^{s}=\phi(\bbx^{s})$, allowing movement between high probability areas. Moving along the manifold can then be neatly achieved by using a distribution membership test based on the kernel Maximum Mean Discrepancy (MMD) statistic~\cite{fortet1953convergence,gretton2012kernel}. We use the MMD witness function to find a location $\bbz^t$ close to $\bbz^s$ with high likelihood of label $y^t$. As our mapping from images to convolutional features is irreversible, we solve a small optimization problem to recover $\bbx^t$ such that $\phi(\bbx^t)\approx \bbz^t$. 

%The first challenge above can be addressed by extracting approximate low-dimensional data manifold. In this paper, we utilize a deep convolutional representation~\cite{simonyan2014very} that has been trained on 1.2 million natural images from the ImageNet corpus~\cite{ILSVRC15}. We use the feed-forward convolutional network as a mapping onto the manifold, $\phi(\cdot)$. This way, we can map the source image onto the lower-dimensional feature representation, $\bbz^s=\phi(\bbx^s)$.    
%In this paper we observe that we can extract a good approximation of the low-dimensional data manifold of natural images from We use the feed-forward convolutional network as a mapping onto the manifold, $\phi(\cdot)$, and map our source image onto the new feature representation, $\bbz^s=\phi(\bbx^s)$. 

%Once the manifold is captured, 

The resulting algorithm allows us to traverse the manifold of natural images freely in a completely data-driven way. We only require labeled images from the source and target classes, and no hand annotation (e.g., correspondances or strokes).  Our method is able to make general class-specific changes, all that is necessary are labeled source and target images.

While this method certainly does not replace specialized methods, this method may function as a baseline for a wide variety of tasks, or perhaps enable some tasks for which no specialized algorithms have been derived. Our results indicate that our method is highly general and performs better than current general methods (which make use of image morphing) on a number of different tasks.




%Our contributions are: 1. We propose a method to avoid the difficulties faced in \cite{szegedy2013intriguing} by proposing a transformation objective function beyond changing an image's label under a discriminative model. 2. We demonstrate empirically several image tasks where we transform the image in a way that discernibly changes the object label, yet \emph{leaves the original object largely intact}. 

%\Yixuan{We could say additionally something like ``yet keeps the image staying on the underlying manifold''.}


%We advance image label transformation in two key ways. First, we overcome the difficulties faced in \cite{szegedy2013intriguing} by proposing a transformation objective function beyond changing an image's label under a discriminative model. Second, we demonstrate empirically that for several tasks, we are able to transform the objects in an image in a way that changes the label of the image, but transforms the objects in a \emph{meaningful way,} yet \emph{leaves the original object largely intact}.




\iffalse
\begin{figure}[t]
\begin{center}
\vspace{-2ex}
\centerline{
\includegraphics[width=0.6\textwidth]{figures/HFManifold.pdf}
%\includegraphics[width=2.7in]{figures/hillary_bush.pdf}
}
\vspace{-2ex}
\caption{An illustration of several manifold traversals from source images (white border) to various target labels. All target images (black border) are synthetically generated with our method from the respective source images (best viewed in color; zoom in to reveal facial details). The sample target images are represented as colored dots and give rise to the target distribution (orange contours) along the manifold; none of them are from the two subjects. White dots represent ImageNet natural images that were used to learn the global natural images manifold (blue). }
%Privacy and utility for both Spearman's $\rho$ and Kendall's $\tau$.}
%\vspace{-10ex}
\label{fig:ht}
\end{center}
\end{figure}
\fi


==> manifold_fig_text.tex <==
%!TEX root=main.tex
\section{Manifold traversal by varying lambda.}
\label{sec:manifold}


\begin{figure*}[tb]
\begin{center}
%\vspace{-2ex}
\centerline{\includegraphics[width=\textwidth]{figures/ShallowVsDeep.pdf}}
\vspace{-2ex}
\caption{\textbf{(Zoom in for details.)} Several methods used to change the age of an input image of Harrison Ford.}
%Privacy and utility for both Spearman's $\rho$ and Kendall's $\tau$.}
\vspace{-5ex}
\label{fig:ID}
\end{center}
\end{figure*}


==> quantitative.tex <==
%!TEX root=main.tex
\paragraph{Quantitative results.}
\label{sec:quant}

%\begin{wrapfigure}{R}{0.5\textwidth}%[h]
\begin{figure}
\begin{center}
%\vspace{-2ex}
\centerline{\includegraphics[width=\textwidth]{figures/quant_old.pdf}}
\vspace{-2ex}
\caption{(\emph{Left}) How the SVM decision value changes during deep manifold traversal from young to old. For large lambdas, the decision value is negative, indicating the image is classified as a young person. As lambda decreases, the decision value increases and eventually becomes positive, indicating the image is classified as an old person. (\emph{Right}) The same evaluation but for deep manifold traversal from smiling to frowning. After reaching $\lambda\!=\!5 \times 10^{-6}$ the SVM confidently predicts that the image is of a frowning person.}
%Privacy and utility for both Spearman's $\rho$ and Kendall's $\tau$.}
\vspace{-5ex}
\label{fig:quant}
\end{center}
\end{figure}
%\end{wrapfigure}

In Figure~\ref{fig:quant} (\emph{Left}), we quantitatively evaluate whether deep manifold traversal actually changes the classification of an input. The vertical axis shows the decision value of a linear SVM as we increasingly change an input using deep manifold traversal. Here, negative values indicate an SVM prediction of \emph{young} for an input image while positive values correspond to an SVM classification of \emph{old}. This SVM was trained on the activations of conv5\_1 of the VGG network using all of the images in the LFW dataset, except 20 hold-out images. We select these 20 images, which the SVM classified confidently as young with a signed classification score of -2.0, and then traversed from young to old. We tracked the change in SVM decision score ($\bw^\top \bx$) for each image during this traversal (as $\lambda$ decreases). Figure~\ref{fig:quant} shows this change in pictures for one of the 20 images, and with the blue line which shows the average decision score. We found that as we traverse from young to old, the SVM decision score increases to become very positive, indicating the SVM confidently believes the traversed images are old. The error bars (95\% confidence) summarize the results over the 20 images. At $\lambda \!=\! 5 \times 10^{-6}$ the labels of all the images have changed to old. Similarly in Figure~\ref{fig:quant} (\emph{Right}), we train an SVM in the same way to detect smiling versus frowning images. We again plot the decision values of this SVM on 20 held-out images throught traversal from frowning to smiling. As with the previous example we see that as $\lambda$ decreases the SVM classifies the traversed images with high confidence as frowning images.


==> tsne_text.tex <==
%!TEX root=main.tex
\paragraph{t-SNE visualization of image transformations.}
\label{sec:tsne}
We want to visualize the manifold traversal trajectory along with the source and target domains embedded in.
Because we cannot visualize high-dimensional spaces directly we use a prominent visualization technique called t-Stochastic Neighbor Embedding (t-SNE) \cite{van2008visualizing}. t-SNE visualizes high-dimensional datasets in two or three dimensions by learning an embedding such that points are close in the low-dimensional visualization can be indicative of their closeness in the original space.

Figure~\ref{fig:tsne} shows a t-SNE visualization of a subset of the LFW dataset (with 50 ``senior'' faces and 50 non-``senior'' faces, randomly sampled from each category). We track three points along a manifold traversal. The closest neighbors of the input image (denoted in red color) are largely non-``senior'' images. As we traverse the manifold, the neighbors of the learned image become increasingly ``senior''. The trajectory of the manifold traversal is highlighted by the arrows in Figure~\ref{fig:tsne}. The visualization indicates that we are truly traversing a meaningful latent manifold with minimal budget from the source to the target domain during the optimization procedure.


%\begin{wrapfigure}{R}{0.5\textwidth}%[h]
\begin{wrapfigure}{R}{0.5\textwidth}
%\begin{figure}
\begin{center}
%\vspace{-2ex}
\centerline{\includegraphics[width=0.5\textwidth]{figures/tSNE.pdf}}
\vspace{-2ex}
\caption{\textbf{Left:} colored points are locations in the latent low-dimensional PCA space, embedded in two dimensions using t-SNE. Blue points are labeled ``senior'' and green points are non-``senior''. The red points near the center track an input image and three points along a manifold traversal towards the ``senior'' class. \textbf{Right:} a zoomed in view of the boxed region. Arrows indicate the manifold traversal trajectory. Zoom in for details.}
%Privacy and utility for both Spearman's $\rho$ and Kendall's $\tau$.}
%\vspace{-10ex}
\label{fig:tsne}
\end{center}
%\end{figure}
\end{wrapfigure}

